NUV-DoA: NUV Prior-based Bayesian Sparse Reconstruction with Spatial Filtering for Super-Resolution DoA Estimation

Achieving high-resolution Direction of Arrival (DoA) recovery typically requires high Signal to Noise Ratio (SNR) and a sufficiently large number of snapshots. This paper presents NUV-DoA algorithm, that augments Bayesian sparse reconstruction with spatial filtering for super-resolution DoA estimation. By modeling each direction on the azimuth's grid with the sparsity-promoting normal with unknown variance (NUV) prior, the non-convex optimization problem is reduced to iteratively reweighted least-squares under Gaussian distribution, where the mean of the snapshots is a sufficient statistic. This approach not only simplifies our solution but also accurately detects the DoAs. We utilize a hierarchical approach for interference cancellation in multi-source scenarios. Empirical evaluations show the superiority of NUV-DoA, especially in low SNRs, compared to alternative DoA estimators.

==> algorithm.tex <==
%%%%%%%%%%%%%%%%%,
%%% Algorithm %%%
%%%%%%%%%%%%%%%%%
%
\begin{algorithm}
\scriptsize
\setstretch{0.15}
  \KwData{$\gvec{Y},\tilde{\gvec{A}}, K, L$}
  \begin{enumerate}
      \item Initialize: $\gvec{q^{(0)}}=(\gscal{q_1^{(0)}},\cdots,\gscal{q_M^{(0)}})^\top \in \mathbb{R}^M \neq 0$
      \item \While{  $\lVert \gvec{q^{(i+1)}}-\gvec{q^{(i)}}\lVert \geq threshold$ and $i\leq i_{\text{max}}$} 
      {\begin{subequations}
              \begin{align}
                  &\gvec{W}=(\tilde{\gvec{A}}\cdot \diag{(\gvec{q^{(i)}})}^2\cdot \tilde{\gvec{A}}^\herm+ \frac{\sigma^2}{L}\cdot \mathbf{I})^{-1}\\
                  &\gvec{m_x}=\diag{(\gvec{q^{(i)}} )}^2\cdot\tilde{\gvec{A}}^\herm\cdot \gvec{W} \cdot \gvec{y}_{\text{mean}}\\
                  &\gvec{V_x}=(\gvec{q^{(i)})^2} -  \diag{(\gvec{q^{(i)}})}^4 \cdot diagonal(\tilde{\gvec{A}}^\herm\cdot \gvec{W} \cdot \tilde{\gvec{A}})\\
                  &\gvec{(q^{(i+1)})}^2=|\gvec{m_x}|^2 +\gvec{V_x}
              \end{align}
            \end{subequations}}

      \item Estimate the spectrum with the fixed $\gvec{\hat{q}^2}$: 
      %
          \begin{equation}
          |\hat{\gvec{x}}|=|\diag{(\gvec{\hat{q}^2})}\cdot \tilde{\gvec{A}}^\herm\cdot \gvec{W} \cdot \gvec{y_{\text{mean}}}|
          \end{equation}
          %
        \item Sparsified spectrum is obtained by keeping only the largest $K$ peaks. If $|\gscal{\hat{x}_j}|\neq 0$ for some $j$, $\frac{(j-1)\pi}{M} - \frac{\pi}{2}$ is one of our estimated direction.
  \end{enumerate}
  \caption{NUV-EM based SSR.}
    \label{alg: doa nuvem}
\end{algorithm}
